Radio emission from a pulsar's magnetic pole revealed by general relativity

Binary pulsars are affected by general relativity (GR), causing the spin axes of each pulsar to precess. We present polarimetric radio observations of PSR J1906+0746 that demonstrate the validity of the geometrical model of pulsar polarisation. We reconstruct the (sky-projected) polarisation emission map over the pulsar's magnetic pole and predict the disappearance of the detectable emission by 2028. Two additional tests of GR are performed in this system, including the spin-precession for strongly self-gravitating bodies. We constrain the relativistic treatment of the pulsar polarisation model and measure the pulsar beaming fraction, with implications for the population of neutron stars and the expected rate of neutron star mergers.

==> table-global-rvm.tex <==
\begin{table}
\caption{{\bf Geometry of the PSR~J1906$+$0746 system.} Results of the global precession model at a 68 per cent
  confidence level assuming the geometry centred on the MP, and the
  reference epoch in MJD, $T_0=53573$. The first column indicates the
  free parameters included in the model and the second column shows
  the value of the parameters.}
\label{tab:globalRVM}
\begin{center}
\begin{tabular}{lr}

\hline
\multicolumn{1}{c}{Parameter} & Value \\
\hline
Magnetic inclination angle of the MP, $\alpha_{\text{MP}}$ (deg)	& $99.41_{-0.17}^{+0.16}$  \\
Misalignment angle, $\delta$ (deg) 			& $104\pm{9}$\\
Reference precessional phase, $\Phi_{0}$ (deg)		& $249_{-9}^{+10}$\\ 
PA offset, $\Delta \psi_{0}$ (deg)			& $29\pm12$\\
Precession rate, $\Omega_\text{p} $ (deg yr$^{-1}$)     & $2.17_{-0.10}^{+0.11}$ \\
Inclination angle, $i$ (deg)                            & $45_{-2.6}^{+3.1}$\\
\hline

\end{tabular}
\end{center}

\end{table}


==> table-obs2.tex <==
\begin{longtable}{crrcrrrrr}
%\begin{minipage}{130mm}
\caption{Results of the `complex' RVM fitting with \textsc{modelRVM}
  for each of the 13 integrated profiles. The columns show the
  weighted MJD of the integrated profiles, the angle between the
  rotation axis and the magnetic axis of the main pulse
  ($\alpha_{\textrm{MP}}$), the angle between the magnetic axis of the
  main pulse and the closest approach to the line of sight
  ($\beta_{\textrm{MP}}$), the longitude of the RVM fit
  ($\phi_{0_{\textrm{MP}}}$) and the PA value
  ($\psi_{0_{\textrm{MP}}}$). $h_{\textrm{em}}$ indicate the
  corresponding emission height assuming the shift
  $\phi_{0_{\textrm{MP}}}$ is solely due to A/R \cite{bcw91}. The last
  two columns show the $\chi^2$ value and the number of data points
  included in the fit.  The quoted uncertainties represent the 95 per
  cent confidence levels.}
%\begin{center}
%\begin{tabular}{crrcrrrrr}
%\hline

%MJD &
%T$_\textrm{int}$ &
%RM &
%\multicolumn{1}{c}{$\alpha_{\textrm{MP}}$} &
%\multicolumn{1}{c}{$\beta_{\textrm{MP}}$} &
%\multicolumn{1}{c}{$\psi_{0}$} &
%\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{MP}}$} &
%\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{IP}}$} \\ &
%(hr) &
%(rad m$^{-2}$) &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(km)} &
%\multicolumn{1}{c}{(km)}\\
%\hline
%\endfirsthead
%\hline
%\multicolumn{12}{c}%                                                             
%{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\ 
%MJD &
% T$_\textrm{int}$ &
%RM &
%\multicolumn{1}{c}{$\alpha_{\textrm{MP}}$} &
%\multicolumn{1}{c}{$\beta_{\textrm{MP}}$} &
%\multicolumn{1}{c}{$\psi_{0}$} &
%\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{MP}}$} &
%\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{IP}}$} \\ &
%(hr) &
%(rad m$^{-2}$) &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(deg)} &
%\multicolumn{1}{c}{(km)} &
%\multicolumn{1}{c}{(km)}\\
%\hline
%\endhead
%\hline
 53571.9 & 21.5 (53527 - 53615) & 155(7) & \\
 53653.1 & 12.0 (53622 - 53706) & 144(7) & \\
 53752.6 & 6.3 (53718 - 53796) & 153(6) & \\
 53843.5 & 2.3 (53817 - 53874) & 146(7) & \\
 53925.8 & 5.5 (53887 - 53975) & 159(7) & \\
 54023.9 & 3.5 (53987 - 54056) & 147(7) & \\
 54108.4 & 6.6 (54069 - 54156) & 149(6) & \\
 54190.0 & 8.0 (54158 - 54242) & 159(6) & \\ 
 54281.8 & 6.5 (54263 - 54329) & 153(8) & \\
 54444.3 & 10.3 (54351 - 54515) & 136(13) & \\
 54591.0 & 6.0 (54536 - 54626) & 156(7) & \\
 54758.8 & 9.8 (54685 - 54890) & 152(2) & \\
 55024.1 & 9.7 (54917 - 55130) & 155(3) & \\
 56012.4 & 2.1 & 150(2) & \\
 56087.2 & 2.1 & 155(3) & \\
 56145.1 & 2.2 & 156(3) & \\
 56178.0 & 1.8 & 150(3) & \\ 
 56213.9 & 2.2 & 152(3) & \\
 56263.7 & 1.9 & 149(3) & \\
 56311.6 & 2.2 & 157(3) & \\
 56347.5 & 2.2 & 153(3) & \\
 56523.0 & 1.8 & 154(3) & \\
 56583.9 & 2.2 & 162(3) & \\
 56743.4 & 1.6 & 155(3) & \\
 56758.4 & 1.5 & 148(3) & \\
 56788.3 & 2.0 & 149(4) & \\
 56819.2 & 1.9 & 150(4) & \\
 56940.9 & 2.1 & 154(3) & \\
 56962.8 & 2.2 & 154(2) & \\
 57190.2 & 1.7 & 153(4) & \\
 57206.2 & 1.9 & 153(4) & \\
 57310.9 & 2.1 & 158(5) & \\
 57333.8 & 2.1 & 153(6) & \\
 57553.2 & 2.2 & 148(7) & \\
 57712.8 & 1.8 & 157(3) & \\ 
 57755.6 & 1.8 & 153(3) & \\
 57769.6 & 1.4 & 153(3) & \\
 57822.5 & 1.3 & 152(3) & \\ 
 57858.4 & 1.8 & 152(5) & \\ 
 57890.3 & 1.3 & 149(6) & \\
 57921.2 & 2.1 & 152(3) & \\
\hline
%\end{tabular}%
\label{tab:obs}
%\end{center}
%\end{minipage}
\end{longtable}



==> table-observations2.tex <==
\begin{longtable}{lcrllSSS}
\caption{{\bf Summary of the observations.} Summary of the 47 epochs in
  our dataset with the results of the individual RVM and emission
  height analysis. The columns show the MJD of the observation, the
  integration time, the RM measured at each epoch, the magnetic
  inclination axis of the IP, the impact parameter of the IP, the
  derived emission ehight for the MP and IP, respectively. The $^\dag$
  symbol indicates the weighted MJD of all Nan\c cay observations
  averaged together over several weeks to months. The $^\dag$ symbol
  shows that a reliable RVM fit could not be obtained for some epochs
  as the slope of the PA under the IP was almost flat.}
\label{tab:data}
\\
\hline
%PSR JName   & N$_{j}$   & $A_{\text{RN}}$ & $\gamma_{\text{RN}}$ & $A_{\text{DM}}$  & $\gamma_{\text{D\M}}$ & Observatory & Frequency & Year Range  & N$_{\text{TOAs}}$ & $E_f$ & $E_q$ \\
\multicolumn{1}{c}{MJD} &
\multicolumn{1}{c}{Backend} &
T$_\textrm{int}$ &
\multicolumn{1}{c}{RM} &
\multicolumn{1}{c}{$\alpha_{\textrm{IP}}$} &
\multicolumn{1}{c}{$\beta_{\textrm{IP}}$} &
\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{MP}}$} &
\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{IP}}$} \\
&
&
(hr) &
\multicolumn{1}{c}{(rad m$^{-2}$)} &
\multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(km)} &
\multicolumn{1}{c}{(km)}\\
\hline
\endfirsthead
%\multicolumn{12}{crrrrrcccccc}%                                                                       
\multicolumn{7}{c}%                                                                                   
{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\hline
\multicolumn{1}{c}{MJD} &
\multicolumn{1}{c}{Backend} &
T$_\textrm{int}$ &
\multicolumn{1}{c}{RM} &
\multicolumn{1}{c}{$\alpha_{\textrm{IP}}$} &
\multicolumn{1}{c}{$\beta_{\textrm{IP}}$} &
\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{MP}}$} &
\multicolumn{1}{c}{$h_{\textrm{em}_\textrm{IP}}$} \\
 & 
 &
(hr) &
\multicolumn{1}{c}{(rad m$^{-2}$)} &
\multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(km)} &
\multicolumn{1}{c}{(km)}\\
\hline
\endhead
\hline
 53571.9$^\dag$ & BON & 21.5 & 155(7) &   	$80.6_{-0.6}^{+0.5}$ & ${13.1_{-1.1}^{+1.3}}$ &  98(8) & 109(46) \\
 53653.1$^\dag$ & BON & 12.0 & 144(7) &   	$80.8_{-0.8}^{+0.7}$ & ${11.7_{-1.4}^{+1.8}}$ &  114(10) & 52(41) \\
 53752.6$^\dag$ & BON & 6.3 & 153(6) &   	$81.7_{-1.1}^{+0.9}$ & ${10.0_{-1.9}^{+2.5}}$ &  106(8) & 136(39) \\
 53843.5$^\dag$ & BON & 2.3 & 146(7) &   	$80.0_{-2.4}^{+1.5}$ & ${13.1_{-3.2}^{+5.2}}$ &  151(10) & 82(32) \\
 53925.8$^\dag$ & BON & 5.5 & 159(7) &   	$79.5_{-2.2}^{+1.5}$ & ${14.3_{-3.2}^{+4.7}}$ &  143(8) & 106(35) \\
 54023.9$^\dag$ & BON & 3.5 & 147(7) &   	$80.3_{-2.2}^{+1.4}$ & ${12.3_{-2.8}^{+4.6}}$ &  154(9) & 91(46) \\
 54108.4$^\dag$ & BON & 6.6 & 149(6) &   	$79.7_{-1.4}^{+1.1}$ & ${12.4_{-2.1}^{+3.0}}$ &  166(10) & 124(37) \\
 54190.0$^\dag$ & BON & 8.0 & 159(6) &    	$79.3_{-1.5}^{+1.1}$ & ${11.9_{-2.3}^{+3.4}}$ &  173(9) & 102(31) \\
 54281.8$^\dag$ & BON & 6.5 & 153(8) &   	$81.4_{-2.4}^{+1.3}$ & ${10.2_{-2.7}^{+5.4}}$ &  194(10) & 60(54) \\
 56012.4 & PUPPI & 2.1 & 150(2) &   	$79.0_{-0.9}^{+0.8}$ & ${2.8_{-0.1}^{+0.1}}$ &  291(22) & 18(41) \\
 56087.2 & PUPPI & 2.1 & 155(3) &   	$79.6_{-1.2}^{+1.0}$ & ${2.7_{-0.1}^{+0.1}}$ &  271(24) & 6(38) \\
 56145.1 & PUPPI & 2.2 & 156(3) &   	$78.6_{-1.2}^{+1.0}$ & ${2.5_{-0.1}^{+0.1}}$ &  280(23) & 6(37) \\
 56178.0 & PUPPI & 1.8 & 150(3) &    	$79.2_{-1.3}^{+1.1}$ & ${2.2_{-0.1}^{+0.1}}$ &  262(23) & 0(38) \\
 56213.9 & PUPPI & 2.2 & 152(3) &   	$79.5_{-1.1}^{+0.9}$ & ${2.1_{-0.1}^{+0.1}}$ &  224(27) & 0(38) \\
 56263.7 & PUPPI & 1.9 & 149(3) &   	$79.5_{-1.5}^{+1.2}$ & ${1.9_{-0.1}^{+0.1}}$ &  310(29) & 1(40) \\
 56311.6 & PUPPI & 2.2 & 157(3) &   	$80.5_{-1.0}^{+0.9}$ & ${1.7_{-0.1}^{+0.1}}$ &  313(26) & 19(40) \\
 56347.5 & PUPPI & 2.2 & 153(3) &   	$79.4_{-1.2}^{+1.1}$ & ${1.8_{-0.1}^{+0.1}}$ &  283(25) & 8(38) \\
 56523.0 & PUPPI & 1.8 & 154(3) &   	$78.7_{-2.5}^{+1.9}$ & ${0.9_{-0.1}^{+0.1}}$ &  289(28) & 27(45) \\
 56583.9 & PUPPI & 2.2 & 162(3) &   	$79.7_{-2.5}^{+1.6}$ & ${0.6_{-0.1}^{+0.1}}$ &  299(27) & 0(41) \\
 56743.4 & PUPPI & 1.6 & 155(3) &   	{---}$^\ddag$ & {---}$^\ddag$ &  281(31) & 0(54) \\
 56758.4 & PUPPI & 1.5 & 148(3) &   	{---}$^\ddag$ & {---}$^\ddag$ &  298(27) & 38(48) \\
 56788.3 & PUPPI & 2.0 & 149(4) &   	{---}$^\ddag$ & {---}$^\ddag$ &  205(37) & 0(51) \\
 56819.2 & PUPPI & 1.9 & 150(4) &   	{---}$^\ddag$ & {---}$^\ddag$ &  223(29) & 0(53) \\
 56940.9 & PUPPI & 2.1 & 154(3) &   	{---}$^\ddag$ & {---}$^\ddag$ &  315(19) & 0(44) \\
 56962.8 & PUPPI & 2.2 & 154(2) &   	{---}$^\ddag$ & {---}$^\ddag$ &  295(25) & 0(39) \\
 57190.2 & PUPPI & 1.7 & 153(4) &   	$89.6_{-26}^{+0.3}$ & ${-1.4_{-0.1}^{+0.1}}$ &  290(28) & 27(40) \\
 57206.2 & PUPPI & 1.9 & 153(4) &   	$77.6_{-17}^{+8.3}$ & ${-1.6_{-0.1}^{+0.2}}$ &  307(26) & 0(42) \\
 57310.9 & PUPPI & 2.1 & 158(5) &   	$65.6_{-28}^{+24}$ & ${-1.9_{-0.2}^{+0.6}}$ &  265(48) & 0(43) \\
 57333.8 & PUPPI & 2.1 & 153(6) &   	$83.7_{-4.1}^{+2.3}$ & ${-2.0_{-0.1}^{+0.1}}$ &  242(24) & 0(36) \\
 57553.2 & PUPPI & 2.2 & 148(7) &   	$79.8_{-23}^{+6.6}$ & ${-3.2_{-0.2}^{+0.4}}$ &  254(25) & 58(35) \\
 57712.8 & PUPPI & 1.8 & 157(3) &    	$75.7_{-46}^{+7.5}$ & ${-3.8_{-0.3}^{+1.8}}$ &  {---} & 43(38) \\
 57755.6 & PUPPI & 1.8 & 153(3) &   	$88.0_{-5.5}^{+1.9}$ & ${-4.3_{-0.2}^{+0.2}}$ &  {---} & 25(35) \\
 57769.6 & PUPPI & 1.4 & 153(3) &   	$89.5_{-1.8}^{+0.4}$ & ${-4.1_{-0.2}^{+0.2}}$ &  {---} & 7(36) \\
 57822.5 & PUPPI & 1.3 & 152(3) &    	$76.6_{-42}^{+12}$ & ${-4.4_{-0.3}^{+1.7}}$ &  {---} & 48(36) \\
 57858.4 & PUPPI & 1.8 & 152(5) &    	$58.4_{-42}^{+29}$ & ${-3.9_{-0.7}^{+2.6}}$ &  {---} & 39(33) \\
 57890.3 & PUPPI & 1.3 & 149(6) &   	$39.9_{-33}^{+45}$ & ${-3.0_{-1.6}^{+2.4}}$ &  {---} & 93(30) \\
 57921.2 & PUPPI & 2.1 & 152(3) &   	$88.6_{-40}^{+1.3}$ & ${-5.0_{-0.2}^{+1.1}}$ &  {---} & 51(33) \\
 58116.7 & PUPPI & 1.2 & 154(3) & 
\end{longtable}

